Improving FSM State Enumeration Performance for Hardware Security with RECUT and REFSM-SAT

Finite state machines (FSM's) are implemented with sequential circuits and are used to orchestrate the operation of hardware designs. Sequential obfuscation schemes aimed at preventing IP theft often operate by augmenting a design's FSM post-synthesis. Many such schemes are based on the ability to recover the FSM's topology from the synthesized design. In this paper, we present two tools which can improve the performance of topology extraction: RECUT, which extracts the FSM implementation from a netlist, and REFSM-SAT, which solves topology enumeration as a series of SAT problems. In some cases, these tools can improve performance significantly over current methods, attaining up to a 99\% decrease in runtime.

==> figures/uart.tex <==
\begin{figure}
\centering
\begin{tikzpicture}[->,scale=1]

%\draw [help lines] (0,0) grid (8, 4);
%\draw (0, 0) rectangle (7.75,5.25); % outer rect

\node (n000) [circle, draw, minimum size=1.5cm, fill=lightgray] at (3.000,4.000) {IDLE};
\node (n010) [circle, draw, minimum size=1.5cm, fill=lightgray] at (5.023,2.531) {START};
\node (n101) [circle, draw, minimum size=1.5cm, fill=lightgray] at (0.977,2.531) {END};
\node (n011) [circle, draw, minimum size=1.5cm, fill=lightgray] at (4.250,0.153) {BIT};
\node (n100) [circle, draw, minimum size=1.5cm, fill=lightgray] at (1.750,0.153) {NEXT};

\path (n000) edge[black] (n010);
\path (n010) edge[black] (n011);
\path (n011) edge[black] (n100);
\path (n100) edge[black] (n011);
\path (n011) edge[black] (n101);
\path (n101) edge[black] (n000);
\path (n100) edge[red,dashed] (n000);

\path (n000.north) edge[out=90+40,in=90-40,distance=0.75cm] (n000.north);
\path (n010.north east) edge[out=45+40,in=45-40,distance=0.75cm] (n010.north east);
\path (n101.north west) edge[out=135+40,in=135-40,distance=0.75cm] (n101.north west);
\path (n011.south east) edge[out=-45+40,in=-45-40,distance=0.75cm] (n011.south east);
%\path (n100.south west) edge[out=225+40,in=225-40,distance=0.75cm] (n100.south west);

\end{tikzpicture}
\caption{UART FSM with added transition\addressed{~\travis{Does the next state have a self loop?}}}
\label{fig:eviluart}
\end{figure}
